Dual-Camera Joint Deblurring-Denoising

Recent image enhancement methods have shown the advantages of using a pair of long and short-exposure images for low-light photography. These image modalities offer complementary strengths and weaknesses. The former yields an image that is clean but blurry due to camera or object motion, whereas the latter is sharp but noisy due to low photon count. Motivated by the fact that modern smartphones come equipped with multiple rear-facing camera sensors, we propose a novel dual-camera method for obtaining a high-quality image. Our method uses a synchronized burst of short exposure images captured by one camera and a long exposure image simultaneously captured by another. Having a synchronized short exposure burst alongside the long exposure image enables us to (i) obtain better denoising by using a burst instead of a single image, (ii) recover motion from the burst and use it for motion-aware deblurring of the long exposure image, and (iii) fuse the two results to further enhance quality. Our method is able to achieve state-of-the-art results on synthetic dual-camera images from the GoPro dataset with five times fewer training parameters compared to the next best method. We also show that our method qualitatively outperforms competing approaches on real synchronized dual-camera captures.

==> sections/supp_abstract.tex <==
Here, we provide the additional material to the main manuscript with the following outline. In Sec.\ \ref{sec:data}, we elaborate on our synthetic data generation pipeline. We discuss details of noise model and blurry data generation that help simulating long and short exposure images. In Sec.\ \ref{sec:results}, we provide more qualitative examples to compare competitive methods, as well as single-task baselines, on both synthetic and real data. Finally, Sec.\ \ref{sec:arch} outlines details of our network architecture.
